Merge to Learn: Efficiently Adding Skills to Language Models with Model Merging

Adapting general-purpose language models to new skills is currently an expensive process that must be repeated as new instruction datasets targeting new skills are created, or can cause the models to forget older skills. In this work, we investigate the effectiveness of adding new skills to preexisting models by training on the new skills in isolation and later merging with the general model (e.g. using task vectors). In experiments focusing on scientific literature understanding, safety, and coding, we find that the parallel-train-then-merge procedure, which is significantly cheaper than retraining the models on updated data mixtures, is often comparably effective. Our experiments also show that parallel training is especially well-suited for enabling safety features in LMs relative to continued finetuning and retraining, as it dramatically improves model compliance with safe prompts while preserving its ability to refuse dangerous or harmful prompts.

==> 9_ethics.tex <==
\section*{Ethics Statement}

We do not foresee any increased risk by this work. We utilized publicly available (or soon to be publicly available) datasets and evaluations, and our metho

==> tables/heuristics.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{lccccc}
% \toprule
% Model & \multicolumn{1}{l}{Tulu} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Science\\ (Val)\end{tabular}} & \multicolumn{1}{l}{Coding} & \multicolumn{1}{l}{Safety} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Exagg.\\ Refusals\end{tabular}} \\ \midrule
% Llama 2 + Tulu                  & 0.499                    & 0.278                                                                       & 0.376                      & 0.503                      & 0.992                                                                         \\ \midrule
% Llama 2 + Tulu + Science        & 0.506                    & 0.387                                                                       & -                          & -                          & -                                                                             \\
% Llama 2 + Tulu + Safety         & 0.502                    & -                                                                           & -                          & 0.953                      & 0.336                                                                         \\
% Llama 2 + Tulu + Coding         & 0.500                    & -                                                                           & 0.567                      & -                          & -                                                                             \\ \midrule
% Llama Task Arithmetic - Science & 0.503 & 0.348 & - & - & - \\
% Llama Task Arithmetic - Safety & 0.503 & - & - & 0.893 & 0.900 \\
% Llama Task Arithmetic - Coding & 0.510 & - & 0.467 & - & - \\ \midrule
% Tulu Task Arithmetic - Science & 0.467 & 0.308 & - & - & - \\
% Tulu Task Arithmetic - Safety & 0.485 & - & - & 0.973 & 0.732 \\
% Tulu Task Arithmetic - Coding & 0.500 & - & 0.467 & - & - \\ \bottomrule
% \end{tabular}
% \caption{Using dataset weighting \jacobm{shrink table, maybe focus on just science + coding and do safety separately?}}
% \label{tab:heuristics}
% \end{table*}

\begin{table}[t]
\centering
\begin{tabular}{lccccc}
\toprule
\textbf{Model}                           & \textbf{Tulu} & \textbf{Sci.} & \textbf{Coding} \\ \midrule
Llama, Tulu & 49.9 & 27.8 & 37.6 \\ \midrule
Llama, Tulu/Science & 50.6 & 38.7 & - \\
Llama, Tulu/Coding & 50.0 & - & 56.7 \\
\midrule
% Llama T.A. Science (1.0) & 43.1 & 28.9 & - \\
% Llama T.A. Coding (1.0) & 49.1 & - & 49.4 \\
% \midrule
Llama T.A. Science (H) & 50.3 & 34.8 & - \\
% Tulu T.A. Science  & 0.467 & 0.308 & - \\
% Lin. Interp. Science  & 0.488 & 0.339 & - \\
% \midrule
Llama T.A. Coding (H)  & 51.0 & - & 46.7 \\
% Tulu T.A. Coding   & 0.500 & - & 0.467 \\
% Lin. Interp. Coding   & 0.487 & - & 0.459 \\
\bottomrule            
\end{tabular}
\caption{Using dataset weighting, focusing on science and coding. We only show llama TA because it's the best, but we can show the other options in the appendix? Which baselines should we compare against? Right now rows 2 and 3 are single stage training. Also show continued ft, neither, etc? \jacobm{Only showing vs Llama/Tulu might make sense, to say "look, you can merge this in and not lose Tulu perf"}. 1.0 shows adding the full vector and H is our heuristic}
\label{tab:heuristics}
\end{table}

==> tables/safety_heuristics.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Model}                          & \multicolumn{1}{l}{\textbf{Tulu}} & \multicolumn{1}{l}{\textbf{Safety}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{Exagg.}\\ \textbf{Refusals}\end{tabular}} \\
\midrule
Llama, Tulu & 49.9 & 50.3 & 99.2 \\
\midrule
Llama, Tulu/Safety & 50.2 & 95.3 & 33.6 \\
Tulu, Safety & 28.9 & 100.0 & 09.6 \\
Tulu, Tulu/Safety & 45.1 & 96.5 & 29.2 \\
\midrule
Llama T.A. & \textbf{50.3} & 89.3 & \textbf{90.0} \\
% Tulu T.A.  & 0.485 & 0.973 & 0.732 \\
% Lin. Interp. & 0.496 & 0.879 & 0.912 \\
\bottomrule
\end{tabular}
\caption{Using dataset weighting. We see: any direct finetuning on safety tanks exaggerated refusals, and finetuning only on safety quickly leads to overfitting. Merging shows the best tradeoffs vs Tulu unsafe -- we improve safety by nearly 40pts while degrading exaggerated refusals by <10pts. \jacobm{Should we show all baselines or no? All "safety" models here use 100\% of safety, which is a lot. We'll show the full ablation results in the appendix, any worth showing here?} \jacobm{Probably just show \textbf{one} merging method?}}
\label{tab:safety-heuristics}
\end{table}
